Efficient equilibrium-based stress recovery for isogeometric laminated curved structures

This work focuses on an efficient stress recovery procedure for laminated composite curved structures, which relies on Isogeometric Analysis (IGA) and equilibrium. Using a single element through the thickness in combination with a calibrated layerwise integration rule or a homogenized approach, the 3D solid isogeometric modeling grants an inexpensive and accurate approximation in terms of displacements (and their derivatives) and in-plane stresses, while through-the-thickness stress components are poorly approximated. Applying a further post-processing step, an accurate out-of-plane stress state is also recovered, even from a coarse displacement solution. This is based on a direct integration of the equilibrium equations in strong form, involving high order derivatives of the displacement field. Such a continuity requirement is fully granted by IGA shape function properties. The post-processing step is locally applied, which grants that no additional coupled terms appear in the equilibrium, allowing for a direct reconstruction without the need to further iterate to resolve the out-of-balance momentum equation. Several numerical results show the good performance of this approach particularly for composite stacks with significant radius-to-thickness ratio and number of plies. In particular, in the latter case, where a layerwise technique employing a number of degrees of freedom directly proportional to the number of plies would be much more computationally demanding, the proposed method can be regarded as a very appealing alternative choice.

==> cylinder.tex <==
In this section we propose several benchmarks to showcase the effectiveness of the proposed approach. To this extent, we consider a composite cylinder solid under bending and we validate the obtained results against an overkilled $C^0$ layerwise solution, addressing main differences with respect to the presented through-the-thickness integration and homogenized approaches as well as the method sensitivity to parameters of interest (i.e., number
of layers and length-to-thickness ratio).

\subsection{Composite cylinder solid under bending}\label{subsec:cylinder_description}
A solid cross-ply cylindrical shell of total thickness $h$ and made of $N$ orthotropic layers is considered in Figure \ref{fig:quarter_cylinder}. The structure is simply supported at both ends and subjected to transverse sinusoidal loading, $q(X_1,X_2,X_3)$, on the inner surface, while the top surface is traction-free. The thickness of every single layer is set to 1 mm, and the edge length, $L$, is chosen to be $S$ times larger than the total thickness of the laminate. 
\begin{figure}[htbp!]
	\centering
	\scalebox{0.7}{\inputtikz{fig_000}}
	\caption{Quarter of composite cylindrical shell: problem geometry.}
	\label{fig:quarter_cylinder}
\end{figure} 
Layer material parameters taken into account for all the numerical tests are summarized in Table \ref{tab:matproperties} for 0\textdegree-oriented plies, while the considered loading pressure is equal to
\begin{equation}\label{eq:load}
q(X_1,X_2,X_3)=\sigma_0\cos(4\theta)\sin(\dfrac{\pi X_1}{Sh})\,,
\end{equation}
where $\sigma_0 =$ -1 MPa and $\theta=\theta(X_2,X_3)\in[0,\bar{\theta}]=[0,\pi/2]$ is oriented anticlockwise as depicted in Figure \ref{fig:quarter_cylinder}.
Having defined the cylinder radius $r=\sqrt{X_2^2+X_3^3}$, we identify the inner and outer surface respectively as $r_i=\bar{R}-\dfrac{h}{2}$ and $r_o=\bar{R}+\dfrac{h}{2}$, being $r_i$ the internal and $r_o$ the external radius.
\begin{table}[!htbp]
	\caption{Numerical tests material properties for 0\textdegree-oriented layers.} 
	\begin{center}
		\small{
			\begin{tabular}{?c c c c c c c c c?}
				\thickhline 
				$E_{1}$ & $E_{2}$& $E_{3}$ & $G_{23}$ & $G_{13}$ & $G_{12}$ & $\nu_{23}$ & $\nu_{13}$ & $\nu_{12}$\Tstrut\Bstrut\\\hline 
				[MPa] & [MPa] & [MPa] & [MPa] & [MPa] & [MPa]& [-] & [-] & [-]\Tstrut\Bstrut\\\thickhline 
				25 & 1 & 1 & 0.2 & 0.5 & 0.5 & 0.25 & 0.25& 0.25\Tstrut\Bstrut\\\thickhline  
		\end{tabular}}
	\end{center}\label{tab:matproperties}
\end{table}\newline
The simply supported edge conditions are taken as
\begin{equation}
\begin{aligned}
\sigma_{11}=0\;\text{and}\;u_2=u_3=0\;\text{at}\;x_1=0\;\text{and}\;x_1=L\,,\label{eq:DBCs}
\end{aligned}
\end{equation}
while Neumann boundary conditions on the tube inner and outer surfaces are
\begin{subequations}\label{eq:NBCs}
\begin{alignat}{2}
&\sigma_{13}=\sigma_{23}=0 \;\text{and}\;\sigma_{33}=q(x_1,x_2,x_3)\quad&&    \quad\text{at}\sqrt{x_2^2+x_3^3}=r_i\,,\label{eq:NBCs_1}\\
&\sigma_{13}=\sigma_{23}=\sigma_{33}=0\quad&&    \quad\text{at}\sqrt{x_2^2+x_3^3}=r_o\,.\label{eq:NBCs_2}
\end{alignat}
\end{subequations}
Taking advantage of the problem symmetry, we model only a quarter of  cylinder, adding the following further constraints
\begin{subequations}\label{eq:sym_BCs}
\begin{align}
&\sigma_{23}=\sigma_{12}=0\;\text{and}\;u_2=0\;\text{at}\;x_2=0\;,\label{eq:sym_BCs_1}\\
&\sigma_{23}=\sigma_{13}=0\;\text{and}\;u_3=0\;\text{at}\;x_3=0\;.\label{eq:sym_BCs_2}
\end{align}
\end{subequations}
All results are then normalized adopting the below reported expression
\begin{alignat}{2}\label{eq:normalizedresults}
\overline{\sigma}_{ij}=\dfrac{\sigma_{ij}}{\lvert\sigma_0\rvert}\quad&\quad i,j=1,2,3\,.
\end{alignat}

\subsection{Single-element layerwise integration approach results}\label{subsec:layerwise}
In this section, we present and comment several numerical examples which consider a quarter of composite cylindrical shell with $S=50$ made of a cross-ply distribution of 11 layers, namely a 0\textdegree/90\textdegree~stacking sequence. All the presented numerical simulations are post-processed starting from a single-element displacement-based IGA-Galerkin approximation with a special through-the-thickness layerwise integration rule and are obtained employing 20x20 control points, an in-plane degree of approximation $p=q=4$ and an out-of plane one equal to $3$.

As an example, in Figure \ref{fig:LWI_IGAG_stress_pt1_1_l11_S50} we present in the left column the in-plane solution profiles for a sampling point located at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$), obtained using an IGA-Galerkin single element approach with a special layerwise integration rule.
Also, in Figure \ref{fig:LWI_IGAG_stress_pt1_1_l11_S50} the right column
compares the out-of-plane stress state for the same sampling point with and without applying the presented post-processing step (see section \ref{sec:recovery}), showing a remarkable improvement in the solution profiles which, after the recovery is performed, are continuous through-the-thickness as equilibrium states. 

% Galerkin: in-plane & post-processed out-of-plane stresses; case: l2mR = 4, S20, 11lays, p 443, 20 cp
\begin{figure}
	\centering
	\subfigure[Normalized $\sigma_{11}$\label{subfig-1:test11}]{\inputtikz{fig_03_a}}\hfill
	\subfigure[Normalized $\sigma_{13}$\label{subfig-2:test11}]{\inputtikz{fig_03_b}}\\
	\subfigure[Normalized $\sigma_{22}$\label{subfig-3:test11}]{\inputtikz{fig_03_c}}\hfill
	\subfigure[Normalized $\sigma_{23}$\label{subfig-4:test11}]{\inputtikz{fig_03_d}}\\
	\subfigure[Normalized $\sigma_{12}$\label{subfig-5:test11}]{\inputtikz{fig_03_e}}\hfill
	\subfigure[Normalized $\sigma_{33}$\label{subfig-6:test11}]{\inputtikz{fig_03_f}}
	\alep{\caption{Through-the-thickness stress profiles evaluated at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$). Case: tube with length-to-mean radius is equal to 4, 11 layers and length-to-thickness ratio $S=20$ (\ref{blueline} layerwise solution, \ref{blackcircles} single-element approach solution (without post-processing), \ref{redcrosses} post-processed solution).}}
	\label{fig:LWI_IGAG_stress_pt1_1_l11_S20}
\end{figure}

\begin{figure}
	\centering
	\subfigure[Normalized $\sigma_{11}$\label{subfig-1:test11S50}]{\inputtikz{fig_04_a}}\hfill
	\subfigure[Normalized $\sigma_{13}$\label{subfig-2:test11S50}]{\inputtikz{fig_04_b}}\\
	\subfigure[Normalized $\sigma_{22}$\label{subfig-3:test11S50}]{\inputtikz{fig_04_c}}\hfill
	\subfigure[Normalized $\sigma_{23}$\label{subfig-4:test11S50}]{\inputtikz{fig_04_d}}\\
	\subfigure[Normalized $\sigma_{12}$\label{subfig-5:test11S50}]{\inputtikz{fig_04_e}}\hfill
	\subfigure[Normalized $\sigma_{33}$\label{subfig-6:test11S50}]{\inputtikz{fig_04_f}}
	\caption{Through-the-thickness stress profiles evaluated at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$). Case: tube with length-to-mean radius equal to 4, 11 layers and length-to-thickness ratio $S=50$ (\ref{blueline} layerwise solution, \ref{blackcircles} single-element approach solution (without post-processing), \ref{redcrosses} post-processed solution).}
	\label{fig:LWI_IGAG_stress_pt1_1_l11_S50}
\end{figure}
In Figures \ref{fig:LWI_IGAG_samplingS13_l11_S20}-\ref{fig:LWI_IGAG_samplingS33_l11_S20} the out-of-plane stress state profile is recovered sampling the composite cylinder every quarter
of length in both in-plane directions, to show the effect of post-processing at different locations of the solid.
Across all sampled points, the proposed approach accurately captures the 3D stresses in every single layer
when compared to an overkilled layerwise solution (namely, 30x30x11 elements and degree of approximation $p=q=6$ and $r=4$). Also, the model remains accurate at the boundaries satisfies Neumann boundary conditions for transverse shear stresses at
the inner and outer surfaces of the laminate as in Eq.\ \eqref{eq:NBCs} and the symmetry conditions with respect to $\sigma_{13}$ and $\sigma_{23}$ as in Eq.\ \eqref{eq:sym_BCs}.
	\begin{figure}[!htbp]
	\centering
	\inputtikz{fig_04}
	\caption{Through-the-thickness $\bar{\sigma}_{13}$ profiles for several in plane sampling points.
	The length-to-mean radius is equal to 4, $L$ represents the total length of the tube, that for this case is  $L=220\,\text{mm}$ (being $L=S\,t$ with $t=11\,\text{mm}$ and $S=20$), while the number of layers is 11 (\ref{redcrosses} post-processed solution, \ref{blueline} layerwise IGA solution).}
	\label{fig:LWI_IGAG_samplingS13_l11_S20}
\end{figure}
\begin{figure}[!htbp]
	\centering
	\inputtikz{fig_05}
	\caption{Through-the-thickness $\bar{\sigma}_{23}$ profiles for several in plane sampling points.
	The length-to-mean radius is equal to 4, $L$ represents the total length of the tube, that for this case is  $L=220\,\text{mm}$ (being $L=S\,t$ with $t=11\,\text{mm}$ and $S=20$), while the number of layers is 11 (\ref{redcrosses} post-processed solution, \ref{blueline} layerwise IGA solution).}
	\label{fig:LWI_IGAG_samplingS23_l11_S20}
\end{figure}
\begin{figure}[!htbp]
	\centering
	\inputtikz{fig_06}
	\caption{Through-the-thickness $\bar{\sigma}_{33}$ profiles for several in plane sampling points.
	The length-to-mean radius is equal to 4, $L$ represents the total length of the tube, that for this case is  $L=220\,\text{mm}$ (being $L=S\,t$ with $t=11\,\text{mm}$ and $S=20$), while the number of layers is 11 (\ref{redcrosses} post-processed solution, \ref{blueline} layerwise IGA solution).}
	\label{fig:LWI_IGAG_samplingS33_l11_S20}
\end{figure}
\newpage
\alepc{Figures 8-10 should be esported with $S=50$!}
\subsubsection{Parametric study on length-to-thickness cylinder ratio}
In order to further investigate the proposed approach, examples which consider a varying length-to-thickness ratio (i.e., $S=20,30,40,\;\text{and}\;50$) are performed respectively
for 11 and 33 layers, examining an increasing number of degrees of freedom.

In Figure \ref{fig:Gal_conv443_varS} we assess the performance of the isogeometric Galerkin approach coupled with the presented post-processing technique at $(x_1=0.25L, \theta=3\,\bar{\theta}/4)$, adopting the following maximum error definition along the thickness
\begin{alignat}{2}\label{eq:error}
&\text{e}(\sigma_{i3})=\cfrac{\text{max}|\sigma_{i3}^\text{analytic}(\bar{x}_1,\bar{x}_2,x_3)-\sigma_{i3}^\text{recovered}(\bar{x}_1,\bar{x}_2,x_3)|}{\text{max}|\sigma_{i3}^\text{analytic}(\bar{x}_1,\bar{x}_2,x_3)|} \quad&&\quad i=1,2,3\,.
\end{alignat}
The post-processing approach seems to be particularly
suitable for laminates characterized by a significant number of layers.
Moreover, we observe that the modeling error, given by the a-posteriori step, dominates over the approximation one; thus, considering a mesh comprising 20x20 control points seems to be suitable enough to correctly capture the composite solid cylinder behavior.

\begin{figure}[!htbp]
	\centering
	\hspace{-7pt}
	\subfigure[11 layers \label{subfig-1:Gal_errors13_l11_443_varS}]{\inputtikz{fig_07_d}}\hspace{-7pt}
	\subfigure[11 layers \label{subfig-2:Gal_errors23_l11_443_varS}]{\inputtikz{fig_07_e}}\hspace{-7pt}
	\subfigure[11 layers \label{subfig-3:Gal_errors33_l11_443_varS}]{\inputtikz{fig_07_f}}\\
	\hspace{-7pt}
	\subfigure[33 layers \label{subfig-4:Gal_errors13_l33_443_varS}]{\inputtikz{fig_08_d}}\hspace{-7pt}
	\subfigure[33 layers \label{subfig-5:Gal_errors23_l33_443_varS}]{\inputtikz{fig_08_e}}\hspace{-7pt}
	\subfigure[33 layers \label{subfig-6:Gal_errors33_l33_443_varS}]{\inputtikz{fig_08_f}}
	\caption{Maximum relative percentage error evaluation, with respect to an IGA layerwise solution, at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$) for IGA-Galerkin post-processed single-element approach using an in-plane degree of approximation equal to 4 and out-of-plane degree of approximation equal to 3. Different length-to-thickness ratios $S$ are investigated for a number of layers equal to 11 and 33 (Number of in-plane control points: \ref{bluesolidcircle} 10,\ref{blacksolidx} 20,\ref{redsolidcross} 40).}
	\label{fig:Gal_conv443_varS}
\end{figure}
\newpage
\subsection{Single-element homogenized approach results}\label{subsec:homog_res}
In this section we discuss results obtained 
% Collocation new
\begin{figure}
	\centering
	\subfigure[Normalized $\sigma_{11}$\label{subfig-1:Colltest11S20}]{\inputtikz{fig_13_a}}\hfill
	\subfigure[Normalized $\sigma_{13}$\label{subfig-2:Colltest11S20}]{\inputtikz{fig_13_b}}\\
	\subfigure[Normalized $\sigma_{22}$\label{subfig-3:Colltest11S20}]{\inputtikz{fig_13_c}}\hfill
	\subfigure[Normalized $\sigma_{23}$\label{subfig-4:Colltest11S20}]{\inputtikz{fig_13_d}}\\
	\subfigure[Normalized $\sigma_{12}$\label{subfig-5:Colltest11S20}]{\inputtikz{fig_13_e}}\hfill
	\subfigure[Normalized $\sigma_{33}$\label{subfig-6:Colltest11S20}]{\inputtikz{fig_13_f}}
	\caption{Through-the-thickness stress profiles evaluated at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$). Case: tube with length-to-mean radius is equal to 4, 11 layers and length-to-thickness ratio $S=20$ (\ref{blueline} layerwise solution, \ref{blackcircles} single-element approach solution (without post-processing), \ref{redcrosses} post-processed solution).}
	\label{fig:Collexample_sig11S20}
\end{figure}


\begin{figure}
	\centering
	\subfigure[Normalized $\sigma_{11}$\label{subfig-1:Colltest11S50}]{\inputtikz{fig_14_a}}\hfill
	\subfigure[Normalized $\sigma_{13}$\label{subfig-2:Colltest11S50}]{\inputtikz{fig_14_b}}\\
	\subfigure[Normalized $\sigma_{22}$\label{subfig-3:Colltest11S50}]{\inputtikz{fig_14_c}}\hfill
	\subfigure[Normalized $\sigma_{23}$\label{subfig-4:Colltest11S50}]{\inputtikz{fig_14_d}}\\
	\subfigure[Normalized $\sigma_{12}$\label{subfig-5:Colltest11S50}]{\inputtikz{fig_14_e}}\hfill
	\subfigure[Normalized $\sigma_{33}$\label{subfig-6:Colltest11S50}]{\inputtikz{fig_14_f}}
	\caption{Through-the-thickness stress profiles evaluated at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$). Case: tube with length-to-mean radius is equal to 4, 11 layers and length-to-thickness ratio $S=50$ (\ref{blueline} layerwise solution, \ref{blackcircles} single-element approach solution (without post-processing), \ref{redcrosses} post-processed solution).}
	\label{fig:Collexample_sig11S50}
\end{figure}

% whole plate collocation

\begin{figure}[!htbp]
	\centering
	\inputtikz{fig_07}
	\caption{Through-the-thickness $\bar{\sigma}_{13}$ profiles for several in plane sampling points.
		The length-to-mean radius is equal to 4, $L$ represents the total length of the tube, that for this case is  $L=220\,\text{mm}$ (being $L=S\,t$ with $t=11\,\text{mm}$ and $S=20$), while the number of layers is 11 (\ref{redcrosses} post-processed solution, \ref{blueline} layerwise IGA solution).}
	\label{fig:ColsamplingS13}
\end{figure}
\begin{figure}[!htbp]
	\centering
	\inputtikz{fig_08}
	\caption{Through-the-thickness $\bar{\sigma}_{23}$ profiles for several in plane sampling points.
		The length-to-mean radius is equal to 4, $L$ represents the total length of the tube, that for this case is  $L=220\,\text{mm}$ (being $L=S\,t$ with $t=11\,\text{mm}$ and $S=20$), while the number of layers is 11 (\ref{redcrosses} post-processed solution, \ref{blueline} layerwise IGA solution).}
	\label{fig:ColsamplingS23}
\end{figure}
\begin{figure}[!htbp]
	\centering
	\inputtikz{fig_09}
	\caption{Through-the-thickness $\bar{\sigma}_{33}$ profiles for several in plane sampling points.
		The length-to-mean radius is equal to 4, $L$ represents the total length of the tube, that for this case is  $L=220\,\text{mm}$ (being $L=S\,t$ with $t=11\,\text{mm}$ and $S=20$), while the number of layers is 11 (\ref{redcrosses} post-processed solution, \ref{blueline} layerwise IGA solution).}
	\label{fig:ColsamplingS33}
\end{figure}
\newpage% Coll
Convergence plots (Homogenized Collocation degree of approximation equal to $6,6,4$).
%\begin{figure}[!htbp]
%	\centering
%	\hspace{-7pt}
%	\subfigure[11 layers \label{subfig-1:Col_errors13_l11_443_varS}]{\inputtikz{fig_009_d}}\hspace{-7pt}
%	\subfigure[11 layers \label{subfig-2:Col_errors23_l11_443_varS}]{\inputtikz{fig_009_e}}\hspace{-7pt}
%	\subfigure[11 layers \label{subfig-3:Col_errors33_l11_443_varS}]{\inputtikz{fig_009_f}}\\
%	\hspace{-7pt}
%	\subfigure[33 layers \label{subfig-4:Col_errors13_l33_443_varS}]{\inputtikz{fig_010_d}}\hspace{-7pt}
%	\subfigure[33 layers \label{subfig-5:Col_errors23_l33_443_varS}]{\inputtikz{fig_010_e}}\hspace{-7pt}
%	\subfigure[33 layers \label{subfig-6:Col_errors33_l33_443_varS}]{\inputtikz{fig_010_f}}
%	\caption{Maximum relative percentage error evaluation, with respect to an IGA layerwise solution, at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$) for IGA-Collocation post-processed single-element approach using an in-plane degree of approximation equal to 4 and out-of-plane degree of approximation equal to 3. Different length-to-thickness ratios $S$ are investigated for a number of layers equal to 11 and 33 (Number of in-plane control points: \ref{bluedashedcircle} 10,\ref{blackdashedx} 20,\ref{reddashedcross} 40).}
%	\label{fig:Col_conv443_varS}
%\end{figure}

%\begin{figure}[!htbp]
%	\centering
%	\hspace{-7pt}
%	\subfigure[11 layers \label{subfig-1:Col_errors13_l11_664_varS}]{\inputtikz{fig_09_d}}\hspace{-7pt}
%	\subfigure[11 layers \label{subfig-2:Col_errors23_l11_664_varS}]{\inputtikz{fig_09_e}}\hspace{-7pt}
%	\subfigure[11 layers \label{subfig-3:Col_errors33_l11_664_varS}]{\inputtikz{fig_09_f}}\\
%	\hspace{-7pt}
%	\subfigure[33 layers \label{subfig-4:Col_errors13_l33_664_varS}]{\inputtikz{fig_10_d}}\hspace{-7pt}
%	\subfigure[33 layers \label{subfig-5:Col_errors23_l33_664_varS}]{\inputtikz{fig_10_e}}\hspace{-7pt}
%	\subfigure[33 layers \label{subfig-6:Col_errors33_l33_664_varS}]{\inputtikz{fig_10_f}}
%	\caption{Maximum relative percentage error evaluation, with respect to an IGA layerwise solution, at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$) for IGA-Collocation post-processed single-element approach using an degree of approximation equal to 6. Different length-to-thickness ratios $S$ are investigated for a number of layers equal to 11 and 33 (Number of in-plane control points: \ref{bluedashedcircle} 10,\ref{blackdashedx} 20,\ref{reddashedcross} 40).}
%	\label{fig:Col_conv664_varS}
%\end{figure}

\begin{figure}[!htbp]
	\centering
	\hspace{-7pt}
	\subfigure[11 layers \label{subfig-1:Col_errors13_l11_666_varS}]{\inputtikz{fig_11_d}}\hspace{-7pt}
	\subfigure[11 layers \label{subfig-2:Col_errors23_l11_666_varS}]{\inputtikz{fig_11_e}}\hspace{-7pt}
	\subfigure[11 layers \label{subfig-3:Col_errors33_l11_666_varS}]{\inputtikz{fig_11_f}}\\
	\hspace{-7pt}
	\subfigure[33 layers \label{subfig-4:Col_errors13_l33_666_varS}]{\inputtikz{fig_12_d}}\hspace{-7pt}
	\subfigure[33 layers \label{subfig-5:Col_errors23_l33_666_varS}]{\inputtikz{fig_12_e}}\hspace{-7pt}
	\subfigure[33 layers \label{subfig-6:Col_errors33_l33_666_varS}]{\inputtikz{fig_12_f}}
	\caption{Maximum relative percentage error evaluation, with respect to an IGA layerwise solution, at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$) for IGA-Collocation post-processed single-element approach using an in-plane degree of approximation equal to 6 and out-of-plane degree of approximation equal to 4. Different length-to-thickness ratios $S$ are investigated for a number of layers equal to 11 and 33 (Number of in-plane control points: \ref{bluedashedcircle} 10,\ref{blackdashedx} 20,\ref{reddashedcross} 40).}
	\label{fig:Col_conv666_varS}
\end{figure}
\newpage
\subsubsection{Homogenized IGA-Galerkin}
\begin{figure}
	\centering
	\subfigure[Normalized $\sigma_{11}$\label{subfig-1:h2}]{\inputtikz{fig_h2_a}}\hfill
	\subfigure[Normalized $\sigma_{13}$\label{subfig-2:h2}]{\inputtikz{fig_h2_b}}\\
	\subfigure[Normalized $\sigma_{22}$\label{subfig-3:h2}]{\inputtikz{fig_h2_c}}\hfill
	\subfigure[Normalized $\sigma_{23}$\label{subfig-4:h2}]{\inputtikz{fig_h2_d}}\\
	\subfigure[Normalized $\sigma_{12}$\label{subfig-5:h2}]{\inputtikz{fig_h2_e}}\hfill
	\subfigure[Normalized $\sigma_{33}$\label{subfig-6:h2}]{\inputtikz{fig_h2_f}}
	\caption{Through-the-thickness stress profiles evaluated at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$). Case: tube with length-to-mean radius is equal to 4, 11 layers and length-to-thickness ratio $S=50$ (\ref{blueline} layerwise solution, \ref{blackcircles} single-element approach solution (without post-processing), \ref{redcrosses} post-processed solution).}
	\label{fig:h2}
\end{figure}

\begin{figure}[!htbp]
	\centering
	\hspace{-7pt}
	\subfigure[11 layers \label{subfig-1:h}]{\inputtikz{fig_h1_d}}\hspace{-7pt}
	\subfigure[11 layers \label{subfig-2:h}]{\inputtikz{fig_h1_e}}\hspace{-7pt}
	\subfigure[11 layers \label{subfig-3:h}]{\inputtikz{fig_h1_f}}
	\caption{Maximum relative percentage error evaluation, with respect to an IGA layerwise solution, at ($x_1=0.25L$, $\theta=3\,\bar{\theta}/4$) for IGA-Galerkin post-processed single-element approach using an in-plane degree of approximation equal to 4 and out-of-plane degree of approximation equal to 3. Different length-to-thickness ratios $S$ are investigated for a number of layers equal to 11 and 33 (Number of in-plane control points: \ref{bluesolidcircle} 10,\ref{blacksolidx} 20,\ref{redsolidcross} 40).}
	\label{fig:h1}
\end{figure}

\newpage
\alepc{In the Following: table 1 should be assessment of IGA-G vs post-processed IGA-G (LWI) vs post-processed IGA-G (H); table 2 should be assessment of IGA-C vs  post-processed IGA-C (H)}
\begin{table}[!htbp]
	%\caption{Simply supported composite plate under sinusoidal load with a number of layers equal to 11. Out-of-plane stress state maximum relative error with respect to Pagano's solution~\cite{Pagano1970} at $x_1=x_2=0.25L$. Comparing the isogeometric collocation-based homogenized single element approach (IGA-C) and the coupled post-processing technique (IGA-C+PP) for different approximation degrees.} 	\vspace{0.5cm}
	\centering	
	\begin{tabular}{? l | c ? c | c | c ? c | c | c ?}
		\thickhline
		\multicolumn{2}{? c ?}{\textbf{Degree}}
		& \multicolumn{3}{c ?}
		{$p=q=6$, $r=4$}&\multicolumn{3}{c ?}{$p=q=r=6$}\Tstrut\Bstrut\\\thickhline
		\multirow{2}{*}{$\boldsymbol{S}$} &\multirow{2}{*}{\textbf{Method}}
		&e($\sigma_{13}$)
		&e($\sigma_{23}$) 
		&e($\sigma_{33}$) 
		&e($\sigma_{13}$) 
		&e($\sigma_{23}$) 
		&e($\sigma_{33}$)  
		\Tstrut\Bstrut\\\cline{3-8}
		& &[\%]&[\%]&[\%]&[\%]&[\%]&[\%]
		\Tstrut\Bstrut\\\thickhline
		\multirow{2}{*}{20} & IGA-G & 97.6 & 56.7 & 6.34 & 96.6 & 56.1 & 6.31\Tstrut\Bstrut\\
		& IGA-G+PP & 0.31 & 2.94 & 0.90 & 1.97 & 1.20 & 0.05\Tstrut\Bstrut\\\hline
		\multirow{2}{*}{30} & IGA-G & 98.7 & 55.6 & 6.36 & 98.3 & 55.4 & 6.34\Tstrut\Bstrut\\
		& IGA-G+PP & 0.16 & 1.34 & 0.47 & 0.91 & 0.57 & 0.08\Tstrut\Bstrut\\\hline
		\multirow{2}{*}{40} & IGA-G & 99.2 & 55.3 & 6.37 & 98.9 & 55.2 & 6.36\Tstrut\Bstrut\\
		& IGA-G+PP & 0.07 & 0.78 & 0.34 & 0.50 & 0.35 & 0.12\Tstrut\Bstrut\\\hline
		\multirow{2}{*}{50} & IGA-G & 99.4 & 55.1 & 6.38 & 99.2 & 55.1 & 6.38\Tstrut\Bstrut\\
		& IGA-G+PP & 0.03 & 0.52 & 0.29 & 0.30 & 0.25 & 0.15\Tstrut\Bstrut\\\thickhline
	\end{tabular}\label{tab:errorl11}
\end{table}


